Defunctionalization with Dependent Types

The defunctionalization translation that eliminates higher-order functions from programs forms a key part of many compilers. However, defunctionalization for dependently-typed languages has not been formally studied. We present the first formally-specified defunctionalization translation for a dependently-typed language and establish key metatheoretical properties such as soundness and type preservation. The translation is suitable for incorporation into type-preserving compilers for dependently-typed languages

==> Makefile <==
MAIN = defun
LATEXMK=latexmk -pdflatex -bibtex -shell-escape
.PHONY: mk

RULESFILE = ott-rules.tex
AUTOGEN = $(MAIN).mng
AGDAFILES = $(patsubst %.lagda,agda/%.tex,$(wildcard *.lagda))

mk: agda.sty $(AGDAFILES) $(AUTOGEN)
	$(LATEXMK) $(MAIN).mng

agda.sty: $(AGDAFILES)

agda/%.tex: %.lagda
	agda --latex $< --latex-dir=agda

OTT_FILES  = spec/spec.ott
OTT_OPTS  = -tex_show_meta false
WARN_MSG = "%%% !!! WARNING: AUTO GENERATED. DO NOT MODIFY !!! %%%\n"

$(RULESFILE): $(OTT_FILES) short-rule-names.sed
	ott -tex_wrap false -picky_multiple_parses true -signal_parse_errors true  $(OTT_OPTS) -o $@ $<
# 	sed -f short-rule-names.sed -i $(RULESFILE)
	@perl -pi -e 'print $(WARN_MSG) if $$. == 1' $@
	@if grep '<<no parses (' $@ >/dev/null 2>&1 && \
		[ -z "$(DONTSTOP)" ]; then \
			echo; \
			echo "***** OTT PARSE ERROR(S) *****"; \
			grep -n '<<no parses (' $@; \
			$(RM) $@; \
			exit 1; \
	fi >&2

# ott_override.tex: override.tex $(OTT_FILES)
# 	ott $(OTT_OPTS) -tex_filter $< $@ $(OTT_FILES)

%.mng: %.tex $(OTT_FILES) $(RULESFILE)
	ott -picky_multiple_parses true -signal_parse_errors true -tex_wrap false $(OTT_OPTS) -tex_filter $< $@ $(OTT_FILES)

clean:
	latexmk -c defun
	rm -f *.{log,bbl,nav,rev,snm,vrb,vtc} ott-rules.tex

diff: mk
	(cd ../pldi2023-submission && make)
	latexdiff --flatten ../pldi2023-submission/$(MAIN).mng $(MAIN).mng \
           | sed -e '/^%DIFDELCMD < $$/{N;N;s!^%DIFDELCMD < \n\n%DIFDELCMD <!%DIFDELCMD < \n%DIFDELCMD <!}' \
           > diff.tex
	$(LATEXMK) diff

fix:
	rm defun.aux

.PHONY: all clean diff


==> agda/compose_defun_context.tex <==
-- \begin{code}%
\>[0]\AgdaComment{--\ \{-\#\ OPTIONS\ --type-in-type\ \#-\}}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}end\{code\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ \textbackslash{}begin\{code\}}\<%
\\
\>[0]\AgdaComment{--\ data\ Π\ :\ (A\ :\ Set)\ ->\ (A\ ->\ Set)\ ->\ Set}\<%
\\
\>[0]\AgdaComment{--\ \AgdaUnderscore{}\$\AgdaUnderscore{}\ :\ ∀\ \{A\ :\ Set\}\ \{p\ :\ A\ →\ Set\}\ ->\ Π\ A\ p\ ->\ (x\ :\ A)\ ->\ p\ x}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}end\{code\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ \textbackslash{}begin\{code\}[hide]}\<%
\\
\>[0]\AgdaComment{--\ infixl\ 9\ \AgdaUnderscore{}\$\AgdaUnderscore{}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ A\ :\ Set}\<%
\\
\>[0]\AgdaComment{--\ A\ =\ \{!!\}}\<%
\\
\>[0]\AgdaComment{--\ B\ :\ Π\ A\ (\textbackslash{}\AgdaUnderscore{}\ ->\ Set)}\<%
\\
\>[0]\AgdaComment{--\ B\ =\ \{!!\}}\<%
\\
\>[0]\AgdaComment{--\ C\ :\ Π\ A\ (\textbackslash{}x\ ->\ Π\ (B\ \$\ x)\ (\textbackslash{}\AgdaUnderscore{}\ ->\ Set))}\<%
\\
\>[0]\AgdaComment{--\ C\ =\ \{!!\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ \{-\#\ NO\AgdaUnderscore{}POSITIVITY\AgdaUnderscore{}CHECK\ \#-\}}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}end\{code\}}\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}begin\{code\}}\<%
\\
\>[0]\AgdaComment{--\ data\ Π\ \ where}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ F1\ :\ Π\ (Π\ A\ (\textbackslash{}y\ ->\ Π\ (B\ \$\ y)\ (\textbackslash{}z\ ->\ C\ \$\ y\ \$\ z)))\ (\textbackslash{}f\ ->\ }\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ \ \ \ \ Π\ (Π\ A\ (\textbackslash{}x\ ->\ B\ \$\ x))\ (\textbackslash{}g\ ->}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ \ \ \ \ Π\ A\ (\textbackslash{}x\ ->}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ \ \ \ \ C\ \$\ x\ \$\ (g\ \$\ x))))}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ F2\ :\ (f\ :\ (Π\ A\ (\textbackslash{}y\ ->\ Π\ (B\ \$\ y)\ (\textbackslash{}z\ ->\ C\ \$\ y\ \$\ z))))\ →}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ \ \ \ \ Π\ (Π\ A\ (\textbackslash{}x\ ->\ B\ \$\ x))\ (\textbackslash{}g\ ->}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ \ \ \ \ Π\ A\ (\textbackslash{}x\ ->}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ \ \ \ \ C\ \$\ x\ \$\ (g\ \$\ x)))}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ F3\ :\ (f\ :\ (Π\ A\ (\textbackslash{}y\ ->\ Π\ (B\ \$\ y)\ (\textbackslash{}z\ ->\ C\ \$\ y\ \$\ z))))\ →}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ \ \ \ \ (g\ :\ (Π\ A\ (\textbackslash{}x\ ->\ B\ \$\ x)))\ →}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ \ \ \ \ Π\ A\ (\textbackslash{}x\ ->}\<%
\\
\>[0]\AgdaComment{--\ \ \ \ \ \ \ \ \ C\ \$\ x\ \$\ (g\ \$\ x))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{--\ \{-\#\ TERMINATING\ \#-\}}\<%
\\
\>[0]\AgdaComment{--\ F1\ \$\ f\ =\ F2\ f}\<%
\\
\>[0]\AgdaComment{--\ F2\ f\ \$\ g\ =\ F3\ f\ g}\<%
\\
\>[0]\AgdaComment{--\ F3\ f\ g\ \$\ x\ =\ f\ \$\ x\ \$\ (g\ \$\ x)\ }\<%
\\
\>[0]\AgdaComment{--\ \textbackslash{}end\{code\}}\<%


==> agda/dcompose.tex <==
\begin{code}[hide]%
\>[0]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\\
\>[0]\AgdaKeyword{variable}\AgdaSpace{}%
\AgdaGeneralizable{C}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitive{Set}\<%
\end{code}

\begin{code}%
\>[0]\AgdaFunction{dcompose}%
\>[18I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{y}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{z}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaBound{y}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{C}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{y}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{z}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{g}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaGeneralizable{B}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaGeneralizable{A}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
\>[18I][@{}l@{\AgdaIndent{0}}]%
\>[10]\AgdaGeneralizable{C}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{g}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{dcompose}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{g}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{x}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{g}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\<%
\end{code}

